Domain-Specific Retrieval-Augmented Generation Using Vector Stores, Knowledge Graphs, and Tensor Factorization

Large Language Models (LLMs) are pre-trained on large-scale corpora and excel in numerous general natural language processing (NLP) tasks, such as question answering (QA). Despite their advanced language capabilities, when it comes to domain-specific and knowledge-intensive tasks, LLMs suffer from hallucinations, knowledge cut-offs, and lack of knowledge attributions. Additionally, fine tuning LLMs' intrinsic knowledge to highly specific domains is an expensive and time consuming process. The retrieval-augmented generation (RAG) process has recently emerged as a method capable of optimization of LLM responses, by referencing them to a predetermined ontology. It was shown that using a Knowledge Graph (KG) ontology for RAG improves the QA accuracy, by taking into account relevant sub-graphs that preserve the information in a structured manner. In this paper, we introduce SMART-SLIC, a highly domain-specific LLM framework, that integrates RAG with KG and a vector store (VS) that store factual domain specific information. Importantly, to avoid hallucinations in the KG, we build these highly domain-specific KGs and VSs without the use of LLMs, but via NLP, data mining, and nonnegative tensor factorization with automatic model selection. Pairing our RAG with a domain-specific: (i) KG (containing structured information), and (ii) VS (containing unstructured information) enables the development of domain-specific chat-bots that attribute the source of information, mitigate hallucinations, lessen the need for fine-tuning, and excel in highly domain-specific question answering tasks. We pair SMART-SLIC with chain-of-thought prompting agents. The framework is designed to be generalizable to adapt to any specific or specialized domain. In this paper, we demonstrate the question answering capabilities of our framework on a corpus of scientific publications on malware analysis and anomaly detection.

==> old_method.tex <==
In this section we outline our framework, explain curation on highly-domain-specific corpus, KG ontology and VS using this corpora, and finally the RAG system. 

\subsection{Domain Specific Dataset}
\todo[inline]{here talk about how we collect the dataset using core documents, citation network, SME keyworks, etc. Then talk about pruning strategies to make sure the core dataset remains good/clean. Pruning strategies are based on removing documents in lower dimension based on distance metrics -- bunnie. emphasize how dataset remains "clean" -- again like in the bunnie paper. tell us about pre-processing techniques used. remember, we need to reference the figures as we describe things.}

Here we define the term ``highly-domain-specific" and explain our dataset collection method. A key feature of our dataset collection is the use of unsupervised methods \cite{TELF} to decompose corpora into document clusters to finer specificity than the author-provided tags available on open access websites. This differs significantly from prior approaches \cite{ABUSALIH2021103076, edwards2024hybrid, yu2022biosalgorithmicallygeneratedbiomedical}. We leverage latent-topic information from our SeNMFk method \cite{Vangara2020} 
% implemented in our \textbf{T}ensor \textbf{E}xtraction of \textbf{L}atent \textbf{F}eatures software, \textbf{T-Elf} \footnote{\url{https://github.com/lanl/T-ELF}}, 
to filter and select the best data for our knowledge base, and prune documents based on citation information and embedding distances. Our text cleaning pipeline is informed by subject matter experts (SME)  \cite{10460022}, thus going beyond standard methods by incorporating expert-derived rules for document cleaning, e.g, acronym and entity standardization. 


The extraction of the latent structure from the data set is accomplished through the following systematic and detailed approach. Initially, the data is prepared and the necessary computational framework is established through the following steps:
\begin{itemize}
 \item The tensor object that contains the cleaned corpus is created.
 \item The cleaned texts is decomposed using \textbf{T-Elf}, improved with the %our new 
 binary search strategy \cite{barron2024binarybleedfastdistributed}, to classify the documents into topic-clusters.
\end{itemize}

Final cluster counts are based on achieving the highest silhouette scores above a predetermined threshold using the Binary Bleed method. This method employs a binary search strategy across \( k \) values, selectively skipping those \( k \) values that do not surpass the silhouette threshold. The search criterion for an optimal \( k \) is defined as \( k_{\text{optimal}} = \max \left\{ k \in \{1, 2, \ldots, K\} : S(f(k)) > T \right\} \), where \( S(f(k)) \) denotes the silhouette score of the \( k \)-th configuration and \( T \) the threshold. Importantly, even after identifying an initial 'optimal' \( k \), our method continues to explore higher \( k \) values to ensure no better configuration is overlooked.

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{figures/KG_only_revised.pdf}
     \vspace{-2em}
    \caption{  The knowledge graph schema aggregated from structured data. Nodes labels are Document, Author, NERs (Event, Person, Location, Product, Organization, Geopolitical Entity), Publisher, Acronyms, SME Keywords, Affiliation, Affiliation Country, Year, \textbf{T-Elf} Topic, \textbf{T-Elf} Keywords. Images generated with DALL·E \cite{dalle_tensor_decomp_arxiv_images}. }
    \label{fig:KG}
\end{figure}

\subsection{Dimension Reduction}
\todo[inline]{here talk about NMFk and what kind of features it allows us to extract from the highly specific data. tell us about post-processing techniques used to clean data and also extract features.}

\subsection{Knowledge Graph Ontology}
\todo[inline]{here talk about how document metadata as well as NMFk latent features are used for out KG. tell us about the KG nodes and edges.}

At a minimum, the development of knowledge graphs requires building a corpus, defining an ontology, and extracting the relevant entity-relation triplets from unstructured text. 

Our ontology is shaped by traditional methods, i.e., relying on SME design and capturing task-specific features. However, we innovate by incorporating latent information from our decomposition process \cite{TELF} into our KG as entities. For entity and relation extraction, we move beyond conventional learning-based techniques \cite{ji2022}; and instead, leverage recent advancements which use LLM-agents \cite{Liu_LlamaIndex_2022, ye2023isolationmultiagentsynergyimproving} as opposed to other LLM prompting methods \cite{wadhwa-etal-2023-revisiting, marinov2024relation, zavarella2024a, edge2024localglobalgraphrag}. This approach yields non-sparse KGs, meaning, the average out-degree of entities \cite{lv-etal-2020-dynamic, HoGRN} is high. To our knowledge, no prior work integrates all of these methods into their knowledge graph construction process.

The data output produced by \textbf{T-Elf} is structured data, unified from the three data sources: OSTI \cite{osti_website}, SCOPUS \cite{scopus_website}, and Semantic Scholar (S2) \cite{semantic_scholar_website}. This data can be mapped into a sequence of head, entity, and tail relations, a directional triplet. These relations are injected into Neo4j \cite{neo4j2023}. Several rows may relate to a particular node, but are not duplicated due to the 'Match' keyword in Neo4j processing as a set operator.  The primary source of information in the knowledge graph is derived from the documents, which are injected into the graph along with a series of related information as attributes. The in-node document information includes DOI, title, abstract, and source API document identifiers. In addition to the documents, labels include authors (of documents), year (document publication), Scopus category, affiliations, affiliation country, acronyms, publisher, the \textbf{T-Elf} topic, topic keywords, citations, references, and a subset of named entity recognition (NER) entities produced from spaCy's NER labels \cite{spacyEnCoreWebTrf}. The NER labels include events, persons, locations, products, organizations, and geopolitical entities.

\subsection{Vector Store Assembly}
\todo[inline]{here do not talk about the specific dataset as we are not in the results section, just mention how we use document metadata to create a VS and it allows us to preserve semantics}

To augment the RAG, we also introduced a vector database for the original documents using Milvus \cite{2021milvus}. Additionally, a subset of the documents full-text were also vectorized and incorporated into the vector store. 
On average, approximately 5\% of the papers in   datasets have   full-texts available. Once extracted, the full-texts are segmented into smaller paragraphs, each assigned an integer ID to indicate its position within the original document. These paragraphs are then vectorized through the same embedding model to be ingested into the vector store to support the RAG process. The RAG application can query the vector store to find relevant paragraph chunks from these full-texts. If the retrieved text contains the information needed, the LLM can answer the posed question and include a citation of the document, and even more precisely the exact paragraph containing the information. If further information that is related to the paragraph chunk is needed, the application can use the metadata (DOI, author, etc) to expand its search through the knowledge graph.

\subsection{SMART-SLIC RAG}

\todo[inline]{putting it all together now. tell us how KG and VS are using with React Agent as a RAG and how it can use cypher, fine correct nodes edges, as well is reference source with DOI.}

For an LLM agent to reliably deliver accurate real-world information, it is crucial that the relevant data is readily accessible within the system. This access is contingent upon the presence of the necessary data within the designated retrieval sources, namely the KG and the vector store. To populate these resources effectively, data must be meticulously collected and structured from diverse sources. The coherent and reasoned output provided by the LLM is the culmination of these systematic preparatory steps, which are elaborated upon below:

\begin{enumerate}
    \item Data Collection: Gathering comprehensive data from varied sources to ensure a broad and representative dataset.
    \item Data Structuring: Organizing the collected data into a structured format suitable for integration into the KG and vector store.
    \item Data Integration and Accessibility: Ensuring that the LLM can seamlessly access this structured data during its operational phase to produce informed outputs.
\end{enumerate}

These steps are essential for the LLM to function optimally and provide outputs that are both accurate and relevant to user queries.
% \section{Results}
\subsection{ Dataset Construction}
Following the data collection, a specialized cleaning pipeline %, documented in \cite{TELF}, 
was applied to ensure the data's usability and integrity. The cleaning procedures involved the following removals and standardization:
\begin{itemize}
    \item Exclude non-English texts, copyright statements, and various non-essential elements such as stop phrases, formulas, and email addresses.
    \item Remove formatting artifacts like next-line markers, parentheses, brackets, and special characters.
    \item Filter out non-ASCII characters and boundaries, HTML tags, stop words, and standalone numbers.
    \item Eliminate extra whitespace and words $\leq$ two characters.
    \item Standardize punctuation variations, particularly hyphens.
    \item Normalize text to ensure consistency.
\end{itemize}

These meticulous pre-processing cleaning and standardization efforts are essential for preparing the dataset for further analysis, thereby enhancing the quality and consistency of the data.\\



\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/Rag_piepline.pdf}
    \vspace{-1em}
    \caption{  The RAG pipeline. Images generated with DALL·E \cite{dalle_tensor_decomp_arxiv_images}. }
    \label{fig:RAG}
\end{figure}

RAG is an advanced technique in NLP that combines retrieval-based and generation-based methods to enhance response accuracy and relevance. RAG operates by first retrieving pertinent information from an external knowledge base in response to an input query. This retrieved data is then utilized to inform and improve the generative model's outputs, resulting in more precise and contextually relevant responses. By integrating these approaches, RAG addresses the limitations of purely generative models and provides a dynamic, adaptable framework suitable for applications demanding detailed and current information. Figure \ref{fig:RAG} demonstrates the data pipeline utilized throughout this work. The process begins with a user query, which the LLM then uses to query the knowledge graph. The LLM transforms the query into a vector embedding. This embedding is compared to existing texts to find the most similar language. The retrieved information is appended to the original query, and the LLM produces a relevant answer in addition to its training data. Finally, the LLM constructs a final organized answer in natural language to explain the answer to the user's question.


In addition to incorporating the state-of-the-art techniques, we improve our RAG pipeline by modifying our retrieval method to use K-Nearest Neighbors with the Levenshtein metric instead of cosine distance as an entry point for context search. We also construct a ``highly-domain-specific" knowledge base for targeted QA tasks.

To leverage the full potential of RAG, it is crucial to accurately understand the user's question. Our RAG approach includes multiple potential routes depending on a user's question.  The question routing pipeline may be characterized as follows:

\begin{enumerate}
    \item \textbf{Specific Document Query}
        \begin{enumerate}
            \item \textit{ReAct Agent Process}
        \end{enumerate}
    \item \textbf{General Query}
    \begin{enumerate}
            \item \textit{Retrieved Query}
            \item \textit{Synthesized Query}
    \end{enumerate}
\end{enumerate}
Understanding the question results in routing the information contained therein to the correct tool-set and subsequent process.

\textbf{1) Specific Document Query:} If a user's question requires information from a specific document's text (title + abstract), it is better suited for a traditional RAG application in which the LLM interacts with a vector store to find the needed text. In our case, we use a ReAct agent where the vector store search is the sole tool, allowing the LLM to make multiple search requests as required. Specifically, a ReAct agent means the LLM has distinct steps for reasoning and acting after determining the input meaning. The agent receives a modified prompt from the standard ReAct prompt and tools to interact with two databases, Neo4j \cite{neo4j2023} and Milvus \cite{2021milvus}, to reduce the LLM's hallucinations. These databases are wrapped as tools and made available to the agent. We use langgraph \cite{langgraph} to define an execution graph with three nodes, as illustrated in Figure \ref{fig:RAG_diagram}: (1) the ReAct agent, (2) the tool executor, and (3) the end.  

\textit{1.a) ReAct Agent Process:}  The agent node is the central part of the ReAct graph, where the LLM calls are encapsulated. The ReAct agent is responsible for collecting inputs, making actionable decisions, and explaining the results. The prompt to the agent contains four parts:

\begin{enumerate}[label=\alph*.]
     \item General ReAct Instructions 
     \item User Query
     \item Tool Names, Associated Tool Data
     \item A Tool Scratchpad
\end{enumerate}

General instructions inform the agent on how to answer a user's query, including formulating the answer and using tools. The user query helps the agent choose the correct tool or form a direct answer, depending on the robustness of the selected model, such as GPT-4. The tools have specific descriptions and parameters required for their calls, including schemas if interacting with databases. The scratchpad serves as temporary storage for tool calls, responses, and the LLM's reasoning, allowing the agent to iteratively solve complex problems.

The tool executor takes the tool name and input parameters from the agent node, routes to the corresponding function, and returns the output. It handles execution logistics, error handling, logging, and status updates. 

The end node signals that the Reason-Act loop has completed. The final output from the LLM after the retrieval augmented generation is returned to the user. This concludes the RAG process.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/ReAct.pdf}
    \vspace{-2em}
    \caption{ The three execution graph nodes, and the three tools routed from the executor for the ReAct RAG agent. Images generated with DALL·E \cite{dalle_tensor_decomp_arxiv_images}.}
    \label{fig:RAG_diagram}
\end{figure}

\textbf{2) General Query:}  If the user asks a broader question, such as those about trends, the required information is found within the KG. In this route, we start with a preprocessing step in which the LLM performs  NER to decouple specific data from the genericized question. After this, we send the genericized query to a smaller vector store containing pairs of cypher queries and descriptions of the information they return, with embedding vectors generated from the descriptions. From here, there are two possible subroutes. 

\textit{2.a) Retrieved Query:} If one of the retrieved queries returns information that can answer the question, we execute that query before a final LLM call to return the result. If none of the retrieved queries can answer the question, we synthesize a new cypher query.

\textit{2.b) Synthesized Query:} If the LLM takes the "synthesis" route, it uses the graph's schema and the retrieved example queries to generate a new cypher query. To make this process more reliable, we have the LLM audit the generated query. First, we obtain the query's execution plan and profile using the cypher keyword "PROFILE," which provides a list of operators performed on the knowledge graph. We include a description of the relevant low-level operators from Neo4j's official documentation. Once we have this detailed execution plan, we have the LLM perform two steps: first, it translates the execution plan into plain language, then it determines whether it answers the user's question. If the LLM confirms the query is valid, we proceed with the same final step as if we had used a retrieved query instead of a generated one.
